Agonist-Antagonist Pouch Motors: Bidirectional Soft Actuators Enhanced by Thermally Responsive Peltier Elements

In this study, we introduce a novel Mylar-based pouch motor design that leverages the reversible actuation capabilities of Peltier junctions to enable agonist-antagonist muscle mimicry in soft robotics. Addressing the limitations of traditional silicone-based materials, such as leakage and phase-change fluid degradation, our pouch motors filled with Novec 7000 provide a durable and leak-proof solution for geometric modeling. The integration of flexible Peltier junctions offers a significant advantage over conventional Joule heating methods by allowing active and reversible heating and cooling cycles. This innovation not only enhances the reliability and longevity of soft robotic applications but also broadens the scope of design possibilities, including the development of agonist-antagonist artificial muscles, grippers with can manipulate through flexion and extension, and an anchor-slip style simple crawler design. Our findings indicate that this approach could lead to more efficient, versatile, and durable robotic systems, marking a significant advancement in the field of soft robotics.

==> sections/05_discussion.tex <==




One of the primary limitations in the development of thermo-active phase change soft actuators pertains to the influence of gravity on the actuation process. In the locomotion designs, for instance, the effects of gravity were observed to impact the efficiency and consistency of actuation, suggesting that the placement and orientation of Peltier elements may require optimization to mitigate these effects.






%In applications involving the use of a fluid like Novec 7000 within a flexible enclosure, attention must be given to the sealing methods and the mechanisms of heat transfer. For instance, when using a heat seal created with an iron, it's critical to maintain an appropriate distance from the encapsulated fluid to prevent its vaporization and subsequent loss during the sealing phase. Furthermore, after the enclosure is sealed, should there be a concentration of Novec at the bottom while heating is applied from above, the heat needs to traverse the enclosure material or the internal air before causing the fluid to vaporize.















%This paper demonstrates the utility of Peltier devices being integrated to thermo-active soft actuators for active cooling and increased bandwidth. However, there are still many considerations and shortcomings to implementing Peltier technology, which will be discussed alongside the strengths below.

%After running thermal graphs on each Peltier, it was found that optimal current would be around 35\% of max current for 15-20 seconds. This will keep the power from being too high from the internal resistance increasing as the Peltier is heated. Any longer or using more current eliminates the Peltier’s capability for active cooling without an external cooling source. The Peltier’s active time can be increased by utilizing heatsinks, but the heatsinks will still accumulate heat that must be dissipated, removing the Peltier’s capability of active cooling. Therefore, to decrease the amount of time the Peltier needs to be powered, the heat transfer to the actuator must be improved. There is a possibility that this issue could be mitigated by using the Peltiers in a cold environment, drastically reducing the need for active cooling.

%One of the main issues with the heat transfer of the solid silicone actuator was the low thermal conductivity of silicone, along with the Novec-7000 air bubbles expanding within. The silicone expanding creates pockets of air that further reduce the thermal conductivity of the silicone body. This low conductivity resulted in the heating of the soft actuator to be heavily concentrated at the contact surface of the Peltier, which causes localized expansion at the Peltier junction interface. This results in the solid silicone not fully actuating when thicker than around 4mm. Previous studies utilizing resistive heating \cite{Decroly2021-xo,Miriyev2017-ps} experience this problem on a smaller level, as the soft body is built around the axis of an inner coil, and the heating/expansion occurs radially. This finding led to much lower aspect ratios with relation to the Peltier surface for the application design. A possible solution is implementing thermally conductive nanoparticles which would increase the thermal conductivity, leading to shorter heating cycles and further elongation. A working solution to keep the silicone pressed against the Peltier is to apply pressure on the silicone, which is counterproductive when trying to get the silicone to actuate. Some minor success was found by simply tying the silicone to the Peltier using thin metal wire or by binding the silicone to the Peltier with Sil-Poxy. A possible solution would be to create planar surfaces along the actuator that cannot expand for the heating interface.




%The hollow silicone design improved upon the solid silicone design in three ways. First Novec-7000 was injected into the hollow silicone body, removing the need for it to soak for 2 hours in Novec-7000 before being ready to actuate. This design could be further improved with a valve system to continually inject Novec-7000 to maintain a consistent amount of Novec-7000 inside the hollow silicone. Secondly, the design allowed for the Peltier to only need to heat through a thin 1mm membrane of silicone in order to vaporize the Novec-7000, substantially increasing the actuation speed. Thirdly, due to the Novec-7000 being inside the hollow center of the structure, the silicone was less permanently deformed after multiple actuations, and overall has a substantial increase in deactuation speed.

%The hollow silicone design was even further improved by making use of the TEGway Flexible Peltier, and embedding it in the design. The flexible nature of this Peltier allows it to be placed inside of a McKibben muscle and still be considered a soft actuator. Embedding the Peltier, allows for the Peltier to be in direct contact with the Novec-7000, and the opposing side of the Peltier to be open to the air to maintain a similar ability to defuse heat as the non embedded design. This design benefits from not having to heat through a 1mm silicone membrane as well as no longer worrying about the silicone structure pulling away from the Peltier during actuation.

%We were able to create simplistic structures using the thin-membrane design for the applications. The general principle lets the user direct expansion through the introduction of design parameters such as strain-limiting layers.

%In conclusion, the design choice of using a hollow silicone structure to store the phase-change fluid removed the poor thermal conductivity if silicone, increased the longevity of the Novec-7000 in order of hours opposed to minutes, vastly increased the user’s ability to rejuvenate the silicone structure, allows for the actuator to be soft, and removed the need to adhere an expanding silicone body to a Peltier. Additionally, it simplified the application designs to resemble pneumatic soft actuators.

%Overall, Peltiers are inefficient once the power source is removed, as both the hot side and cold side begin to equalize as they are exposed to the ambient temperature. This paper focuses on the Peltier effect, but there may also be applications in soft robotics where the opposite effect, the Seebeck effect, may be beneficial such as energy harvesting \cite{Zadan2022-fl}.

%This study demonstrates the promising implementation of Peltier devices as the heating stimuli of thermo-active soft actuators, which can allow for active cooling and enhanced control.
%Future works include optimization of design and heating, and targeting thermoelectric devices that utilize organic materials, which could be integrated to soft actuators. Additionally, a control system should be integrated for the Peltiers, as heat transfer becomes more efficient if you incorporate the passive heating of the Peltier after current is removed for the actuation process. 


